Constrained episodic reinforcement learning in concave-convex and knapsack settings

We propose an algorithm for tabular episodic reinforcement learning with constraints. We provide a modular analysis with strong theoretical guarantees for settings with concave rewards and convex constraints, and for settings with hard constraints (knapsacks). Most of the previous work in constrained reinforcement learning is limited to linear constraints, and the remaining work focuses on either the feasibility question or settings with a single episode. Our experiments demonstrate that the proposed algorithm significantly outperforms these approaches in existing constrained episodic environments.

==> app_linear_regression.tex <==
% !TEX root = appendix.tex

For constrained linear MDPs, we first provide detailed background for ridge linear regression that is used for estimating the linear MDP's model (transition, reward, and consumptions). We then detour to provide backgrounds on planning using the learned models and discuss computational complexity there (specifically we explain why the computation complexity does not scale with respect to the size of the state space). 

To perform regret analysis, following the regret analysis procedure for tabular setting, we first show that the specific bonus is valid and implies optimistic bonus-enhanced models across all episodes. We then call regret decomposition theorem (Theorem~\ref{thm:regret_decomposition}) together with a lemma that provides the specific form of the upper bounds of the Bellman errors to conclude the proof. 



%\newcommand{\calF}{\mathcal{F}}
\subsection{Qualities of Estimated Models from Ridge Linear Regression}
\label{app:linear_closed_form}
In this section, we derive the prediction error of the learned models from Ridge linear regression. We focus on one particular episode $k$ and hence drop subscript $k$ in the analysis below. 

Recall that the input to ridge linear regression is a dataset $\replay = \{ s_i, a_i, r_i, \vec{c}_i, s'_i\}_{i=1}^N$ that consists of $N$ many tuples and we denote the size of $\replay$ as $| \replay| = N$ here.  The following lemma states the parameterization of the learned $\widehat{\mu}, \widehat{\theta}$ and $\widehat{A}$ and their prediction accuracy. 

Regarding notations in this section, we denote $Y = [ \delta_{s'_1}, \dots, \delta_{s'_N} ]$, $\Phi = [ \phi(s_1,a_i), \dots, \phi(s_N,a_N) ]$, $\vec{r} = [r_1, \cdots, r_N ]^{\top}$, and $C = [ \vec{c}_1,\dots, \vec{c}_N ]$. Also we denote $\phi_i$ in short for $\phi(s_i,a_i)$. Denote $\Lambda = \Phi\Phi^{\top} + \lambda\mathbf{I}$ with $\lambda\in\mathbb{R}^+$. Note that $\Lambda$ is positive definite with the eigenvalues being lower bounded by $\lambda$.

\begin{lemma}[Closed-form solutions of $\widehat\mu, \widehat\theta, \widehat{A}$, norm bounds, computation complexity]
The learned transition $\widehat{\mu}$, reward $\widehat{\theta}$ and consumption functions $\widehat{A}$ has the following closed-form solutions:
\begin{align*}
&\widehat{\mu} = \sum_{i=1}^N \delta_{s'_i} \phi(s_i,a_i)^{\top}\left( \Phi\Phi^{\top}+\lambda\mathbf{I} \right)^{-1},  \widehat\theta = \sum_{i=1}^N \left( \Phi\Phi^{\top} + \lambda\mathbf{I} \right)^{-1} \phi(s_i,a_i) r_i,   \\
& \widehat{A} = \sum_{i=1}^N \vec{c}_i \phi(s_i,a_i)^{\top}\left( \Phi\Phi^{\top} + \lambda\mathbf{I} \right)^{-1}.
\end{align*} Regarding the norms of the learned parameters, we have:
\begin{align*}
\| \widehat{\mu} \| \leq \frac{N}{\lambda}; \quad \|\widehat{\theta}\| \leq \frac{N}{\lambda}, \quad, \| \widehat{A_j}\| \leq \frac{N}{\lambda}, \forall j\in\mathcal{D}.
\end{align*}
Given any function $f:\mathcal{S}\to \mathbb{R}$, regarding computation of $\left(\widehat{\mu}\phi\sa \right) \cdot f$, we have its complexity scales in the order of $O\left( z^2 N + z^{3}\right)$ assume that querying $f(x)$ at any $x$ is $O(1)$. In order to compute $\left(\widehat{\mu}\phi\sa \right) \cdot f$ for any $f$ and any $\sa$, one just needs to store all $N$ data samples (rather than explicitly storing $\widehat{\mu}$). 
\label{lemma:closed_form_solu_linear}
\end{lemma}
\begin{proof} 
The first part of the above lemma can be proven by calling Lemma~\ref{lemma:linear_regression} which states general results for ridge linear regression. 
For the second part, consider $\widehat{\mu}$, we have:
\begin{align*}
\|\widehat{\mu}\| \leq \sum_{i=1}^N \|\delta_{s'_i} \phi_i^{\top} \Lambda^{-1} \| = \sum_{i=1}^N \|\phi_i^{\top} \Lambda^{-1}\| \leq N\frac{1}{\lambda}.
\end{align*} The proof for $\widehat\theta$ and $\widehat{A}_j$ are almost identical. 

Regarding computation $(\widehat{\mu}\phi\sa) \cdot f$, we can write it as:
\begin{align*}
(\widehat{\mu}\phi\sa) \cdot f =  \sum_{i=1}^N \phi\sa^{\top} (\Phi\Phi^{\top}  + \lambda\mathbf{I})^{-1} \phi(s_i, a_i) f(s'_i).
\end{align*} Based on basic linear algebra operation, we can verify that the computation complexity is $O(z^2 N + z^3)$. Also note that if we store all $N$ data points, we do not have to explicitly write down $\widehat{\mu}$ ($\widehat{\mu}$ may have infinite dimension) in order to query $(\widehat{\mu}\phi\sa)\cdot f$ for any given $\sa$ and $f$.  Hence the storage is $O(N)$ assuming each $(s, a, s')$ tuple is $O(1)$.
%Hence the computation includes computing $(\Phi\Phi^{\top} + \lambda\mathbf{I})^{-1}$ of which the complexity is $O(N z^2 + z^3)$, and 


\end{proof}

\begin{lemma}[Prediction Accuracy of $\widehat{\mu}, \widehat{\theta},\widehat{A}$] Fix any $\delta\in (0,1)$.  Denote a discrete function class $\mathcal{F} = \{f: \mathcal{S}\to[0,H]\}$. With probability at least $1-\delta$, we have that for any $\sa$: 
\begin{align*}
&\left\lvert \left(\widehat{\mu} \phi\sa - \mu^\star\phi\sa \right) \cdot f  \right\vert \leq \|\phi\sa\|_{\Lambda^{-1}} \left( \sqrt{\lambda z} H + 2H \sqrt{z\log((N+\lambda)/\lambda)} + 2H \sqrt{\log(|\mathcal{F}|/\delta)}  \right),\\
& \left\lvert (\widehat{\theta} - \theta^\star)\cdot \phi\sa \right\rvert \leq  \sqrt{\lambda} \| \phi\sa\|_{\Lambda^{-1}}, \\
& \left\lvert \left( \widehat{A}_j - A^\star_j \right)\phi\sa  \right\rvert \leq \sqrt{\lambda} \| \phi\sa\|_{\Lambda^{-1}}, \forall j\in \mathcal{D}.
\end{align*}
\label{lemma:model_accuracy}
\end{lemma}
\begin{proof}
We first consider the prediction accuracy of $\widehat{\theta}$.  %For any $\sa$, we can show that:
\begin{align*}
&\widehat{\theta} - \theta^\star =  \sum_{i=1}^N \left( \Phi\Phi^{\top} + \lambda\mathbf{I}\right)^{-1} \phi_i r_i - \theta^\star = \sum_{i=1}^N \left( \Phi\Phi^{\top} + \lambda\mathbf{I}\right)^{-1} \phi_i ( \phi_i^{\top} \theta^\star) - \theta^\star \\
& =  \left( \Phi\Phi^{\top} + \lambda\mathbf{I}\right)^{-1} \Phi\Phi^{\top} \theta^\star - \theta^\star = -\lambda \left( \Phi\Phi^{\top} + \lambda\mathbf{I}\right)^{-1} \theta^\star = -\lambda \Lambda^{-1} \theta^\star.
\end{align*} Hence, for any $\sa$, we have:
\begin{align*}
\left\lvert (\widehat{\theta} - \theta^\star)\cdot \phi\sa \right\rvert \leq \|\theta-\theta^\star\|_{\Lambda^{-1}} \| \phi\sa \|_{\Lambda^{-1}} = \lambda \sqrt{ (\theta^\star)^{\top} \Lambda^{-1} \theta^\star} \|\phi\sa \|_{\Lambda^{-1}}  \leq \sqrt{\lambda} \| \phi\sa\|_{\Lambda^{-1}},
\end{align*} where the first inequality uses Holder's inequality and the last inequality uses the fact that the maximum eigenvalue of $\Lambda^{-1}$ is upper bounded by $1/\lambda$.

Now we consider consumption functions. Denote $\widehat{A}_j$ and $A^\star_j$ as the $j$-th row of $\widehat{A}$ and $j$-th row of $A^\star$ respectively. Following the same derivation above for reward functions, for any $j\in\mathcal{D}$, and any $\sa$, we have that:
\begin{align*}
\left\lvert \left( \widehat{A}_j - A^\star_j \right)\phi\sa  \right\rvert \leq \sqrt{\lambda} \| \phi\sa\|_{\Lambda^{-1}}.
\end{align*}

Now we consider the prediction accuracy of $\widehat{\mu}$. Denote $\widehat{\mu}\phi\sa \cdot f = \sum_{s'\in\mathcal{S}} \widehat{\mu}(s')\phi\sa  f(s')$ where $\widehat{\mu}(s)$ denotes the row of $\widehat{\mu}$ that corresponds to state $s$. 

Use Lemma~\ref{lemma:linear_regression}, we have that with probability at least $1-\delta$, for any $\sa$: 
\begin{align*}
\left\lvert \left(\widehat{\mu} \phi\sa - \mu\phi\sa \right) \cdot f  \right\vert \leq \|\phi\sa\|_{\Lambda^{-1}} \left( \sqrt{\lambda z} H + 2H \sqrt{z\log((N+\lambda)/\lambda)} + 2H \sqrt{\log(|\mathcal{F}|/\delta)}  \right),
\end{align*} where we use the fact that for any $i$, $\|\delta_{s'_i} - \mu\phi_i \|_{1} \leq 2$ when using Lemma~\ref{lemma:linear_regression}.
This concludes the proof of the lemma.
\end{proof}

The above lemma is useful for deriving the form of bonus which allows us to compute optimistic models. 



%\subsection{Planning in MDPs}
%\label{app:linear_plan}




%\wscomment{to do after deadline...}


\subsection{Bonus and Optimism in Linear MDPs}

We are going to focus on episode $k$. We denote $N_k = |\replay_{k-1}|$ the size of the replay buffer used in episode $k$. Recall that we use $\replay_{k-1}$ to perform linear regression to get $\widehat\mu_k, \widehat\theta_k$ and $\widehat{A}_k$.

We consider the following form of bonus $b_k\sa = \beta_k \| \phi\sa  \|_{\Lambda_k^{-1}}$, where  we define the covariance matrix $\Lambda_k = \sum_{\vs,\va \in \replay_{k-1}} \phi(\vs,\va)\phi(\vs,\va)^{\top} + \lambda I$, and set $\beta_k$ as:
\begin{align*}
\beta_k = 8 zH \sqrt{ \log\left(\left(1 + \frac{8 N_k^3 z}{\lambda} \right)\frac{2k^2 (d+1)\mathcal{A}}{\delta}\right) }.
\end{align*}
\paragraph{Value functions for bonus-enhanced models} We focus on episode $k$ and we drop subscript $k$ below in this section. We denote our bonus enhanced model $\mathcal{M} = \left( \widehat{p}, \widehat{r}\sa + b\sa, \{ \widehat{c}(s,a,i) - b\sa \}_{i\in\mathcal{D}} \right)$. Given any policy $\boldpi$, we can compute the value functions in $\mathcal{M}$ as follows. Consider any $m\in \{ r, \mathcal{D} \}$. Starting at $H$, we denote $Q^{\boldpi, p}_{m}(s,a,H) = m\sa$. For any stage $h$, we have:
\begin{align*}
&V^{\boldpi, p}_{m}(s, h+1)  =\max\{0, \min\{ \Exp_{a\sim \boldpi(\cdot|s)} Q^{\boldpi, p}_{m}(s,a, h+1), H\} \}\\
& Q^{\boldpi,p}_{m}(s,a,h) =   m\sa +  p\sa \cdot V_{m}^{\boldpi, p}(s, h+1)    \\
\end{align*} Note that the above equation holds for any $m \in \{r,\mathcal{D}\}$. Now we consider $r$ first. Recall we have $r\sa = \widehat{r}\sa + b_k\sa$ and $p := \widehat{p}$. We have:
\begin{align}
&Q^{\boldpi,p}_{r}(s,a,h) = \widehat{r}\sa + b\sa + \widehat{p}\sa\cdot V_{m}^{\boldpi, p}(s, h+1)\nonumber \\
& = \left( \widehat{\theta} + \sum_{s'\in\mathcal{S}} \widehat{\mu}(s')^{\top} V_{r}^{\boldpi, p}(s', h+1)   \right)\cdot \phi\sa + b\sa  \nonumber \\
& = \left( \widehat{\theta} + \sum_{s'\in\mathcal{S}} \widehat{\mu}(s')^{\top} V_{r}^{\boldpi, p}(s', h+1)   \right)\cdot \phi\sa + \beta \sqrt{ \phi\sa \Lambda^{-1} \phi\sa} \nonumber\\
& := \widehat{w}^{\boldpi, p}_r \cdot \phi\sa + \beta \sqrt{\phi\sa \Lambda^{-1}\phi\sa}.
\label{eq:learned_q}
\end{align}
Similarly, for $c_i$, we have:
\begin{align*}
Q^{\boldpi, p}_{c_i}(s,a, h) =  \widehat{w}^{\boldpi, p}_{c_i}\cdot \phi\sa  - \beta\sqrt{\phi\sa \Lambda^{-1}\phi\sa}.
\end{align*}




\begin{lemma}[Bounds on the parameter $\widehat{w}_m^{\boldpi, p}$] For policy $\boldpi$ and bonus enhance model $p = \widehat{p}, r = \widehat{r} + b$ and $c(s,a,i) = \widehat{c}(s,a,i) - b\sa$, for $Q^{\boldpi, p}_r\sa$ (Eq.~\ref{eq:learned_q}), we have $\| \widehat{w}_m^{\boldpi, p}\| \leq 2HN/\lambda$, for all $m \in \{r, \{c_i\}_{i\in\mathcal{D}}\}$.
\end{lemma}
\begin{proof}
Recall Lemma~\ref{lemma:closed_form_solu_linear}. We have that $\|\widehat{\mu}\| \leq N/\lambda $ and $\|\widehat{\theta}\|\leq N/\lambda$. Hence, for $\widehat{w}^{\boldpi, p}_r$, we have:
\begin{align*}
\| \widehat{w}_r^{\boldpi, p} \| \leq  \| \widehat\theta \| + H \|\widehat{\mu}\| \leq 2H N/\lambda,
\end{align*} where we use the fact that $V^{\boldpi, p}_r(s, h) \in [0,H]$ for any $s, h, \boldpi, p, r$ by construction. 
\end{proof}


%\begin{lemma}[Form of value functions from $\mathcal{M}_k$]
%asdf
%\end{lemma}

\begin{lemma}[$\delta$-valid bonus per episode] Denote the bonus enhanced model as $\mathcal{M} = \{ p, r, \vec{c}\}$ with $p = \widehat{p}$, $r\sa = \widehat{r} + b\sa$ and $c(s,a,i) = \widehat{c}(s,a,i) - b\sa$.  Consider the bonus $b\sa = \xi\sqrt{\phi\sa^{\top}\Lambda^{-1} \phi\sa}$ with $\xi  = 8 z H \sqrt{ \log\left(\left(1 + \frac{8 N^3 z}{\lambda} \right)\frac{A(d+1)}{\delta}\right) }$ With probability at least $1-\delta$, we have that:
\begin{align*}
&\left\lvert ( \widehat{r}\sa - r^\star \sa)  + ( \mu^\star - \widehat{\mu} )\phi\sa \cdot V_{r}^{\boldpi, p}(\cdot, h) \right\rvert \leq b\sa,\\
& \left\lvert ( \widehat{c}(s,a,i) - c^\star(s,a,i))  + ( \mu^\star - \widehat{\mu} )\phi\sa \cdot V_{c_i}^{\boldpi, p}(\cdot, h) \right\rvert \leq b\sa,
\end{align*} for all $s,a$, $\boldpi$, $h$, and all $i\in\mathcal{D}$.%and $m \in \{\hat{r}, \{\hat{c}(\cdot,\cdot,i)\}_{i\in\mathcal{D}}\}$.
\label{lemma:per_episode_bonus}
\end{lemma}
\begin{proof}
We focus on proving the result for $m = r$.  We have:
\begin{align*}
&\left\lvert ( r\sa - r^\star \sa)  + ( \mu^\star - \widehat{\mu} )\phi\sa \cdot V_{r}^{\boldpi, p}(\cdot, h) \right\rvert  \\
&=  \left\lvert (\widehat{\theta}-\theta^\star)\cdot \phi\sa  + ( \mu^\star - \widehat{\mu} )\phi\sa \cdot V_{r}^{\boldpi, p}(\cdot, h)  + b\sa \right\rvert
\end{align*}
Recall Lemma~\ref{lemma:model_accuracy}, we know that for any $\sa$, we have:
\begin{align*}
\left\lvert (\widehat{\theta}-\theta^\star)\cdot \phi\sa \right\rvert \leq \sqrt{\lambda} \|\phi\sa\|_{\Lambda^{-1}}.
\end{align*}
Now we bound the error resulting from model estimation $\widehat\mu$. Fix a particular action $a'\in \mathcal{A}$, and consider the Q function $Q^{\boldpi, \pi}_{r}(s, a, h) = \widehat{w}^{\boldpi, p}_{r} \cdot \phi\sa + \beta \sqrt{\phi\sa^{\top}\Lambda^{-1}\phi\sa}$. Since we know that $\| \widehat{w}_r^{\boldpi, p}\| \leq N /\lambda$, we build an $\epsilon$-net on the following function class:
\begin{align*}
\mathcal{F} = \min\left\{ Q(\cdot ,a'): w^{\top}\phi(\cdot ,a) + \beta\sqrt{\phi(\cdot,a')^{\top}\Lambda^{-1} \phi(\cdot ,a')},H \right\},
\end{align*} with $\|w\| \leq N/\lambda$. Use Lemma~\ref{lemma:epsilon_cover_lemma}, we know that the size of the $\epsilon$-net of $\mathcal{F}$, denote as $\Psi(\mathcal{F})$ is bounded as:
\begin{align*}
\log\left( \Psi(\mathcal{F})\right) \leq z\log(1 + 4 N /  (\lambda\epsilon)) + z^2 \log\left( 1 + 7 z^{0.5} B^2 / (\lambda \epsilon^2) \right).
\end{align*}
Now call Lemma~\ref{lemma:model_accuracy}, we have that with probability at least $1-\delta$,  for any $f\in \Psi(\mathcal{F})$:
\begin{align*}
&\left \| \sum_{i=1}^N \phi_i ( \delta_{s'_i} - \mu^\star\phi_i)\cdot f \right\|_{\Lambda^{-1}} \\
&\quad \leq \underbrace{\left(  \sqrt{\lambda z} H + 2H \sqrt{z\log\left(\frac{N}{\lambda} + 1\right)} +  2H \sqrt{z\log\left(1+\frac{4N}{\lambda\epsilon}\right) - \log\delta} + 2H z\sqrt{\log\left(1 + \frac{7z^{0.5}B^2}{\lambda\epsilon^2}\right) -\log\delta} \right)}_{:= \alpha}.
\end{align*}
Now for any function $f\in \mathcal{F}$, by the definition of $\epsilon$-net, i.e., $\sup_{s} |f(s) - f'(s)| \leq \epsilon$ for some $f'\in\Psi(\mathcal{F})$, we have that:
\begin{align*}
&\left \| \sum_{i=1}^N \phi_i ( \delta_{s'_i} - \mu^\star\phi_i)\cdot f \right\|_{\Lambda^{-1}}  \leq \left \| \sum_{i=1}^N \phi_i ( \delta_{s'_i} - \mu^\star\phi_i)\cdot f' \right\|_{\Lambda^{-1}} + \left \| \sum_{i=1}^N \phi_i ( \delta_{s'_i} - \mu^\star\phi_i)\cdot (f - f') \right\|_{\Lambda^{-1}} \\
& \leq \alpha +  \frac{2\epsilon N}{\lambda}.
\end{align*} Pick $\epsilon = \frac{zH\lambda}{2N}$, we have that:
\begin{align*}
&\alpha + 2\epsilon N /\lambda   \\
& \quad  \leq \underbrace{\sqrt{\lambda z} H + 2H \sqrt{d\log\left(\frac{N}{\lambda} + 1\right)} +  2H \sqrt{z\log\left(1+\frac{8N^2}{\lambda^2 zH}\right)} + 2H z\sqrt{\log\left(1 + \frac{7N^2 z^{0.5}B^2}{\lambda^3 z^2 H^2}\right)} + zH}_{:= \xi}. 
\end{align*}
Note that $\xi \leq 8 zH \sqrt{ \log\left(\left(1 + \frac{8 N^3 z}{\lambda} \right)\frac{1}{\delta}\right) }$.
Hence, for $\left\lvert  (\widehat{\mu} - \mu^\star)\phi\sa \cdot f  \right\rvert $, we have that for any $f\in\mathcal{F}$,
\begin{align*}
\left\lvert  (\widehat{\mu} - \mu^\star)\phi\sa \cdot f  \right\rvert  \leq \xi \|  \phi\sa \|_{\Lambda^{-1}},
\end{align*} which indicates that for $Q^{\boldpi, p}_{r}(\cdot ,a')$, we have:
\begin{align*}
\left\lvert  (\widehat{\mu} - \mu^\star)\phi\sa \cdot Q^{\boldpi, p}_{r}(\cdot ,a)  \right\rvert  \leq \xi \|  \phi\sa \|_{\Lambda^{-1}},
\end{align*} for any $\boldpi, h$ and $\mathcal{M}$. 

Apply a union bound over all actions $\mathcal{A}$, we get that with probability at least $1-|\mathcal{A}| \delta$, 
\begin{align*}
\left\lvert  (\widehat{\mu} - \mu^\star)\phi\sa \cdot Q^{\boldpi, p}_{r}(\cdot ,a)  \right\rvert  \leq \xi \|  \phi\sa \|_{\Lambda^{-1}},
\end{align*} for all $\boldpi, a, \mathcal{M}, h$. Now consider $V^{\boldpi, p}_r(\cdot)$. We have that $V^{\boldpi, p}_r(s) = \sum_{a} \boldpi(a|s) Q^{\boldpi, p}_r(s,a)$, based on the inequality above, we naturally have:
\begin{align*}
-\xi \|\phi\sa\|_{\Lambda^{-1}} \leq (\widehat{\mu} - \mu^\star)\phi\sa \cdot V^{\boldpi, p}_r(\cdot) \leq \xi\|\phi\sa\|_{\Lambda^{-1}}.
\end{align*}

We can repeat similar analysis for each consumptions.  Apply a union bound over rewards and $d$ many consumptions, and over all actions, we conclude the proof. 

%Adjusting failure probability $\delta$ concludes the proof. 

%\begin{align*}
%&\left\lvert  (\widehat{\mu} - \mu^\star)\phi\sa \cdot f  \right\rvert \leq \| \phi\sa \|_{\Lambda^{-1}}\left( \sqrt{\lambda d} H + 2H \sqrt{d\log(N/\lambda + 1)} + 2H \sqrt{ \log(|\Psi(\mathcal{F})|/\delta)}\right) \\
%& \leq  \| \phi\sa \|_{\Lambda^{-1}} \underbrace{\left(  \sqrt{\lambda d} H + 2H \sqrt{d\log\left(\frac{N}{\lambda} + 1\right)} +  2H \sqrt{d\log\left(1+\frac{4N}{\lambda\epsilon}\right)} + 2H d\sqrt{\log\left(1 + \frac{7d^{0.5}B^2}{\lambda\epsilon^2}\right)} \right)}_{:= \alpha}.
%\end{align*}
%Now for any function $f\in \mathcal{F}$, by the definition of $\epsilon$-net, i.e., $\sup_{s} |f(s) - f'(s)| \leq \epsilon$ for some $f'\in\Psi(\mathcal{F})$, we have that:
%\begin{align*}
%&\left\lvert (\widehat{\mu} - \mu^\star)\phi\sa \cdot f \right\rvert \leq \left\lvert (\widehat{\mu} - \mu^\star)\phi\sa \cdot f' \right\rvert +  \| (\widehat{\mu} - \mu^\star)\phi\sa\|_{1} \| f- f'\|_{\infty}\\
%& \leq \alpha \|\phi\sa\|_{\Lambda^{-1}} + N\epsilon /\lambda.
%\end{align*} 

\end{proof}

\begin{lemma}[$\delta$-valid bonus] Denote $\beta_k = 8 zH \sqrt{ \log\left(\left(1 + \frac{8 N_k^3 z}{\lambda} \right)\frac{2 k^2 (d+1)\mathcal{A}}{\delta}\right) }$ and set bonus $b_k\sa = \beta_k \| \phi\sa \|_{\Lambda_k^{-1}}$.  With probability at least $1-\delta$, we have that for any $\boldpi$, and any episode $k$ with bonus-enhanced model $\mathcal{M}_k = (p_k, r_k, \{c_k(\cdot,\cdot, i)_{i\in\mathcal{D}}\})$ with $ (p_k, r_k, \{c(\cdot,\cdot,i)\}_{i\in\mathcal{D}}) =(\widehat{p}_k, \widehat{r}_k\sa + b_k\sa, \{\widehat{c}(s,a,i)_k - b_k(s,a)\}_{i\in\mathcal{D}})$, and any $i\in\mathcal{D}$, we have:
\begin{align*}
&\left\lvert ( \widehat{r}_k\sa - r^\star \sa)  + ( \mu^\star - \widehat{\mu}_k )\phi\sa \cdot V_{r_k}^{\boldpi, p}(\cdot, h) \right\rvert \leq b_k\sa,\\
& \left\lvert ( \widehat{c}_k(s,a,i) - c^\star(s,a,i))  + ( \mu^\star - \widehat{\mu}_k )\phi\sa \cdot V_{c_k(\cdot,\cdot,i)}^{\boldpi, p_k}(\cdot, h) \right\rvert \leq b_k\sa,
\end{align*}
\label{lemma:valid_bonus_linear}
\end{lemma}
\begin{proof}
From Lemma~\ref{lemma:per_episode_bonus}, we know that for a fixed episode $k$, with $\xi  = 8 z H \sqrt{ \log\left(\left(1 + \frac{8 N_k^3 z}{\lambda} \right)\frac{A(d+1)}{\delta}\right) }$ With probability at least $1-\delta$, we have that:
\begin{align*}
\left\lvert ( m_k\sa - m^\star \sa)  + ( \mu^\star - \widehat{\mu}_k )\phi\sa \cdot V_{m_k}^{\boldpi, p_k}(\cdot, h) \right\rvert \leq \xi \|\phi\sa\|_{\Lambda_k^{-1}},
\end{align*} for all $s,a$, $\boldpi$, $h$, and $m \in \{r, \{c(\cdot,\cdot,i)\}_{i\in\mathcal{D}}\}$.  To prove the lemma, we allocate failure of probability $6\delta/(\pi^2k^2)$ to each episode and then apply a union bound over all episodes $k \in\mathbb{N}^+$ with the fact that $\sum_i 6/(i^2\pi^2) = 1$ and inequality $\pi^2/6 \leq 2$.
\end{proof}



\begin{lemma}[Optimism of $\mathcal{M}_k$] Denote $\mathcal{M}_k =\left( \widehat{p}_k, \widehat{r}_k\sa + b_k\sa, \{\widehat{c}_k(s,a,i) - b_k\sa\}_{i\in\mathcal{D}} \right)$ with $b_k\sa$ being $\delta$-valid bonus (i.e., Lemma~\ref{lemma:valid_bonus_linear} holds). We have $\mathcal{M}_k$ being optimistic (Definition~\ref{defn:optimistic_model}) for any episode $k$.
\label{lemma:optimism_linear}
\end{lemma}
\begin{proof}
We prove optimism by induction. We drop subscript $k$ in the proof as we only focus on episode $k$ here.  We also only focus on proving optimism for reward and the proof for consumptions are almost identical.  

We start from $H+1$.  We denote $Q^{\boldpist, p}_r(s,a, H+1) = Q^{\boldpist, p^\star}_{r^\star}(s,a, H+1) = 0$. We assume the inductive hypothesis $Q^{\boldpist, p}_r(s,a, h+1) \geq Q^{\boldpist, p^\star}_{r^\star}(s,a, h+1)$ for all $\sa$.  We now move to time step $h$. We have:
\begin{align*}
&Q^{\boldpist, p}_r(s,a, h) -  Q^{\boldpist, p^\star}_{r^\star}\sa = r\sa + p\sa\cdot V^{\boldpist, p}_{r}(\cdot, h+1) - r^\star\sa - p^\star\sa \cdot V^{\boldpist, p^\star}_{r^\star}(\cdot,h+1)  \\
& = \left( r\sa - r^\star\sa \right) + \left( p\sa - p^\star\sa \right)\cdot V_{r}^{\boldpist, p}(\cdot, h+1)  \\
& \qquad + p^\star\sa \cdot ( V_r^{\boldpist, p}(\cdot, h+1) - V_{r^\star}^{\boldpist, p^\star}(\cdot, h+1)) \\
& \geq \left( r\sa - r^\star\sa \right) + \left( p\sa - p^\star\sa \right)\cdot V_{r}^{\boldpist, p}(\cdot, h+1)  \\
& =  (\widehat{\theta} - \theta^\star)\cdot \phi\sa + \left( \left(\mu^\star - \widehat{\mu}\right)\cdot \phi\sa \right)\cdot V_{r}^{\boldpist, p}(\cdot, h+1) + b\sa,
\end{align*} where in the first inequality we use the inductive hypothesis. 

Recall our assumption that $b$ is $\delta$ valid, i.e., we have with probability at least $1-\delta$, for any $\sa$:
\begin{align*}
\left\lvert (\widehat{\theta} - \theta^\star)\cdot \phi\sa + \left( \left(\mu^\star - \widehat{\mu}\right)\cdot \phi\sa \right)\cdot V_{r}^{\boldpist, p}(\cdot, h+1) \right\rvert \leq b\sa.
\end{align*}  Conditioned on the above event, we have that:
\begin{align*}
&Q^{\boldpist, p}_r(s,a, h) -  Q^{\boldpist, p^\star}_{r^\star}\sa \geq 0, \forall \sa. 
\end{align*} Hence, we complete the proof.
\end{proof}

\subsection{Bounding Bellman errors}
Given $\mathcal{M}_k = (p_k, m_k)$ and any policy $\boldpi$, recall the Bellman error  is defined as:
\begin{align*}
\bellman_{m}^{\boldpi,p}(s,a,h)=
Q_{m}^{\boldpi,p}(s,a,h)-({m^{\star}(s,a)+\sum_{s'\in\states}p^{\star}(s'|s,a)V_{m}^{\boldpi,p}(s',h+1)}).
\end{align*} 
Next, we bound Bellman error. 
\begin{lemma}[Bounding Bellman error] With probability at least $1-\delta$, for any episode $k$, any $\boldpi$, any $s, a, h$, and $m_k\in \{ r_k, \{ c_k(\cdot,\cdot,i)\}_{i\in\mathcal{D}} \}$ and from the bonus-enhanced model $\mathcal{M}_k = (\widehat{p}_k, \widehat{r}_k + b_k\sa, \{\widehat{c}_k(\cdot,\cdot,i) - b_k\sa\}_{i\in\mathcal{D}})$, we have:
\begin{align*}
\left\lvert \bellman_{m_k}^{\boldpi,p_k}(s,a,h) \right\rvert \leq  2 b_k\sa.
\end{align*}
\label{lemma:bellman_upper_bound}
\end{lemma}
\begin{proof}
We start from the definition of bellman error under a bonus enhanced model:
\begin{align*}
&Q_{m_k}^{\boldpi,p_k}(s,a,h)-({m^{\star}(s,a)+p^{\star}(\cdot |s,a)\cdot V_{m_k}^{\boldpi,p_k}(\cdot,h+1)}) \\
& = (m_k\sa  - m^\star\sa) + \left( \widehat{p}_k\sa - p^\star\sa \right)\cdot V^{\boldpi, p_k}_{m_k}(\cdot, h+1)
\end{align*} 
Recall lemma~\ref{lemma:valid_bonus_linear}, we know that with probability at least $1-\delta$, we have that:
\begin{align*}
&\left\lvert ( \widehat{r}_k\sa - r^\star \sa)  + ( \mu^\star - \widehat{\mu}_k )\phi\sa \cdot V_{r_k}^{\boldpi, p}(\cdot, h) \right\rvert \leq b_k\sa,\\
& \left\lvert ( \widehat{c}_k(s,a,i) - c^\star(s,a,i))  + ( \mu^\star - \widehat{\mu}_k )\phi\sa \cdot V_{c_k(\cdot,\cdot,i)}^{\boldpi, p_k}(\cdot, h) \right\rvert \leq b_k\sa.
\end{align*}
Conditioned on this $\delta$-valid bonus event being true, we have that:
\begin{align*}
&\left\lvert (r_k\sa  - r^\star\sa) + \left( \widehat{p}_k\sa - p^\star\sa \right)\cdot V^{\boldpi, p_k}_{r_k}(\cdot, h+1)\right\rvert \\
& \leq b_k\sa + \left\lvert (\widehat{r}_k\sa  - r^\star\sa) + \left( \widehat{p}_k\sa - p^\star\sa \right)\cdot V^{\boldpi, p_k}_{r_k}(\cdot, h+1)   \right\rvert \leq 2b_k\sa. 
\end{align*}
The proof for consumption $c_k$ is almost identical. 
\end{proof}

\subsection{Final regret computation}

%We first use the following lemma to bound the difference between the relevant values of empirical trajectories generated from the sequence of policies and the values from taking the expectation with respect to the policies.

Note regret decomposition theorem (Theorem~\ref{thm:regret_decomposition}) is derived without assuming any structures on the MDP. Hence, Theorem~\ref{thm:regret_decomposition} also holds in constrained Linear MDPs setting. This means that in order to bound the final regret, we just need to upper bound the sum of Bellman errors. 

%Now we are ready to prove the main theorem. 
\begin{proof}[Proof of Theorem~\ref{thm:main_theorem_linear}]
From Lemma~\ref{lemma:optimism_linear} we know that with probability $1-\delta$, $\mathcal{M}_k$ is optimistic for all $k$. 
Recall Theorem~\ref{thm:regret_decomposition}.  We know that the at any episode, if the cMDP $\mathcal{M}_k$ is optimistic, we have the total regret that corresponds to reward being upper bounded as:
\begin{align*}
\sum_{k=1}^K \Exp^{\boldpi_k}\left[ \sum_{h=1}^H \bellman_{r_k}^{\boldpi_k, p_k}(\vs(h),\va(h), h) \right]. 
\end{align*} Note that we have $| \bellman_{r_k}^{\boldpi_k, p_k}(\vs(h),\va(h), h)| \leq 3H$ due to the construction of $Q^{\boldpi, p}_{m}(\cdot, \cdot, h) \in [0, H]$.  Apply Lemma~\ref{lemma:expectation_to_realization}, we know that with probability at least $1-\delta$, we have:
\begin{align*}
\left\lvert\sum_{k=1}^K \Exp^{\boldpi_k}\left[ \sum_{h=1}^H \bellman_{r_k}^{\boldpi_k, p_k}(\vs(h),\va(h), h) \right] -\sum_{k=1}^K \sum_{h=1}^H \bellman_{r_k}^{\boldpi_k,p_k}(s\kh,a\kh) \right\rvert \leq H^{1.5} \sqrt{2\ln(4K^2 /\delta) K}.
\end{align*}
Now we use the upper bound of $\bellman$ derived in Lemma~\ref{lemma:bellman_upper_bound}. We have:
\begin{align*}
&\sum_{k=1}^K \sum_{h=1}^H \bellman_{r_k}^{\boldpi_k,p_k}(s\kh,a\kh) \leq \sum_{k=1}^K \sum_{h=1}^H 2 b_k(s\kh, a\kh) \leq \sum_{k=1}^K \sum_{h=1}^H 2 \beta_k \|\phi(s\kh,a\kh)\|_{\Lambda_{k}^{-1}} \\
& \leq 2 (\max_{k} \beta_k) \sum_{k=1}^K \sum_{h=1}^H \|\phi(s\kh,a\kh)\|_{\Lambda_{k}^{-1}}\leq 2(\max_k \beta_k)  H \sqrt{2 K z \log(1 + KH)},
\end{align*} where we call lemma~\ref{lemma:log_det_lemma} with $\lambda = 1$. 


Note  $\max_k \beta_k \leq 8 z H \sqrt{\log\left( \left( 1+ 8K^3H^3 z \right)\left( 2K^2 (d+1)A \right)/\delta \right)}$. Combine the above result, we have:
\begin{align*}
&\sum_{k=1}^K \Exp^{\boldpi_k}\left[ \sum_{h=1}^H \bellman_{r_k}^{\boldpi_k, p_k}(\vs(h),\va(h), h) \right] \leq H^2 \sqrt{2\ln(4K^2 /\delta) K } + \sum_{k=1}^K \sum_{h=1}^H \bellman_{r_k}^{\boldpi_k,p_k}(s\kh,a\kh) \\
& \leq H^2 \sqrt{2\ln(4K^2 /\delta) K } + 16 z H^2 \sqrt{\log\left( \left( 1+ 8K^3H^3 z \right)\left( 2K^2 (d+1)A \right)/\delta \right)2Kz \log(1+KH)}\\
& \leq 17 H^2 \sqrt{ z^3 K \log\left( \left( 1+ 8K^3H^3 z \right)\left( 2K^2 (d+1)A \right)/\delta \right)2 \log(1+KH)}.
\end{align*}

Following similar derivation for consumptions $c_k$, we conclude the proof. 

\end{proof}




\begin{lemma}Consider episodes from $k = 1$ to $K$. In each episode, we have a sequence of $H$ vectors $\phi\kh$ with $h\in [H]$ and $\|\phi\kh\|\leq 1$ for any $k, h$. Denote $\Lambda_0 = \lambda \mathbb{I}$ with $\lambda \in [0,1]$. Denote $\Lambda_{k} = \Lambda_{k-1} + \sum_{h=1}^H \phi\kh\phi\kh^{\top}$.  We have:
\begin{align*}
\sum_{k=1}^K \sum_{h=1}^H \sqrt{ \phi\kh\Lambda_{k-1}^{-1}\phi\kh} \leq H \sqrt{ 2 K d\log(1+ KH/\lambda)}.
\end{align*}
\label{lemma:log_det_lemma}
\end{lemma}
\begin{proof}
Note by assumption $\Lambda_0$ has minimum eigen-value no smaller than $1$, and $\|\phi\|\leq 1$, we have:
\begin{align*}
\phi^{\top} \Lambda_k^{-1} \phi \leq 1, \forall k.
\end{align*}
From episode $k-1$ to $k$, we have $\Lambda_k = \Lambda_{k-1} + \sum_{h=1}^H \phi\kh\phi\kh^{\top}$. By matrix inverse lemma, we have:
\begin{align*}
\det( \Lambda_{k} ) = \det(\Lambda_{k-1} + \sum_{h=1}^H \phi\kh\phi\kh^{\top} ) = \det(\Lambda_{k-1}) \det\left( \mathbf{I} + \Lambda_{k-1}^{-1/2} \left( \sum_{h=1}^H \phi\kh\phi\kh^{\top}\right) \Lambda_{k-1}^{-1/2} \right).
\end{align*} Note that we have:
\begin{align*}
 \det\left( \mathbf{I} + \Lambda_{k-1}^{-1/2} \left( \sum_{h=1}^H \phi\kh\phi\kh^{\top}\right) \Lambda_{k-1}^{-1/2} \right) = 1 + \sum_{h=1}^H \phi\kh \Lambda_{k-1}^{-1} \phi\kh.
\end{align*} 
Also note that for any $x\in [0,1]$, we have that $\log(1+x) \leq x \leq 2\log(1+x)$, which implies that:
\begin{align*}
\log\left(1 + \sum_{h=1}^H \phi\kh\Lambda_{k-1}^{-1} \phi\kh / H \right) \leq \sum_{h=1}^H \phi\kh \Lambda_{k-1}^{-1} \phi\kh / H \leq 2\log\left(1 + \sum_{h=1}^H \phi\kh\Lambda_{k-1}^{-1} \phi\kh / H \right).
\end{align*} So, we have:
\begin{align*}
\sum_{k=1}^K \sum_{h=1}^H \phi\kh^{\top}\Lambda_{k-1}^{-1} \phi\kh / H \leq 2 \sum_{k=1}^K \log\left(1 + \sum_{h=1}^H \phi\kh\Lambda_{k-1}^{-1} \phi\kh / H \right) = \log\det(  \Lambda_k ) - \log\det(\Lambda_0).
\end{align*} Now use the fact that the maximum eigenvalue of $\Lambda_k$ is at most $\lambda + kH$, we have:
\begin{align*}
\sum_{k=1}^K \sum_{h=1}^H \phi\kh^{\top}\Lambda_{k-1}^{-1}\phi\kh \leq 2H\left( \log\det(\Lambda_{K}) - \log\det(\lambda\mathbf{I})  \right) \leq 2H d\log\left( 1 + KH/\lambda \right).
\end{align*}Now apply Cauchy-Schwartz, we have:
\begin{align*}
\sum_{k=1}^K \sum_{h=1}^H \sqrt{ \phi\kh\Lambda_{k-1}^{-1}\phi\kh} \leq \sqrt{KH} \sqrt{\sum_{k=1}^K \sum_{h=1}^H \phi\kh\Lambda_{k-1}^{-1}\phi\kh}  \leq \sqrt{ 2H^2 K d\log(1+ KH/\lambda)}.
\end{align*}
\end{proof}


%\subsection{Planning in bonus-enhanced models and the computation complexity of value iteration}
\subsection{Computational complexity of value iteration in bonus-enhanced models}

Recall the setting in Lemma~\ref{lemma:closed_form_solu_linear}. Given a model $\calM = (\widehat{p}, \widehat{r}\sa + b\sa)$ where $\widehat{p}\sa = \widehat{\mu}\phi\sa$ and $\widehat{r}\sa = \widehat\theta \cdot\phi\sa$ with $\widehat{\mu}$ and $\widehat{\theta}$ from Lemma~\ref{lemma:closed_form_solu_linear}, and bonus $b\sa$ is in the form of $\beta\sqrt{\phi\sa^{\top} \Lambda^{-1} \phi\sa}$, we can perform value iteration in computation time that scales polynomially with respect to $N, z, |\mathcal{A}|, H$. 
\begin{lemma}
With $\widehat{\mu}, \widehat{\theta}$ learned based on Lemma~\ref{lemma:closed_form_solu_linear}, we have that the computation complexity of value iteration on the bonus enhanced model $(\widehat{p}, \widehat{r} + b)$ scales $\text{poly}(N, z, H, |\mathcal{A}|)$ (no explicitly dependency on size of the state space $\states$).
\end{lemma}
\begin{proof} We proceed by induction. 

Starting from $H$, denote $Q(s,a, H) = \widehat{\theta}\cdot\phi\sa + \beta \sqrt{\phi\sa^{\top}\Lambda^{-1}\phi\sa}$. Namely, $Q(s,a,H)$ is a quadratic function with respect to $\phi\sa$. Given any $\sa$, querying $Q(s,a, H)$ has computation complexity $O(z^2)$.

Assume that $Q(s,a, h+1) = w_{h+1}\cdot \phi\sa + \beta \sqrt{\phi\sa^{\top} \Lambda^{-1} \phi\sa}$.    We proceed to $h$ as follows. 

Note that $V(s, h+1) = \max_{a}Q(s,a, h+1)$ and given any $s$, querying $V(s, h+1)$ requires at most $O(z^2 |\mathcal{A}|)$ computation complexity. For $Q(s,a, h)$, we have:
\begin{align*}
&Q(s,a, h) = \widehat{r}\sa + b\sa + \widehat{P}\sa \cdot V(\cdot, h+1) \\
& = \widehat{\theta} \cdot \phi\sa + \beta\sqrt{\phi\sa^{\top} \Lambda^{-1}\phi\sa } + (\widehat{\mu}\phi\sa) \cdot V(\cdot, h+1)\\
& = \underbrace{\left( \widehat{\theta} + \sum_{s'\in\states}\widehat{\mu}(s')^{\top} V(s', h+1)    \right)}_{w_h}\cdot \phi\sa + \beta\sqrt{\phi\sa^{\top} \Lambda^{-1}\phi\sa},
\end{align*}where $\widehat\mu(s)$ denote a row vector of $\widehat{\mu}$ that corresponds to state $s$. Denote $\overline{\mathcal{S}} = \{s\in\mathcal{S}: \exists i\in [N], s'_i = s\}$ as the collection of the unique states that appear in the dataset $\mathcal{B}$.  Note that $|\overline{\mathcal{S}}| \leq N$.   We can compute $w_h$ as:
\begin{align*}
&\sum_{s\in\states}\widehat{\mu}(s)V(s, h+1) = \sum_{s\in \states} \sum_{i=1}^N \one\{s_i' = s\} \left(\Phi\Phi^{\top} + \lambda\mathbf{I}\right)^{-1}\phi(s_i,a_i) V(s, h+1) \\
& = \sum_{s\in \overline{\mathcal{S}}}V(s, h+1) \sum_{i=1}^N \one\{s_i' = s\} \left(\Phi\Phi^{\top} + \lambda\mathbf{I}\right)^{-1}\phi(s_i,a_i),
\end{align*} which means that the computation complexity of $\sum_{s\in\states}\widehat{\mu}(s)V(s, h+1) $ is $O(Nz^2 + z^3 + N^2 z^2 + Nz^2 |\mathcal{A}|)$, i.e., the computation complexity does not scale with state space size explicitly.  Hence computing $w_h = \widehat{\theta} + \sum_{s\in\states}\widehat{\mu}(s)V(s, h+1) $ has complexity poly in $N$ and $z$ as well. 

With $Q(s,a,h) = w_h\cdot\phi\sa + \beta\sqrt{\phi\sa^{\top}\Lambda^{-1}\phi\sa}$, note that querying $V(s, h)$ takes $O( z^2 |\mathcal{A}| )$ computation complexity.  Hence, via induction, we can compute $\{ w_h \}_{h=1}^H$ with computation complexity
\begin{align*}
\text{poly}(N, z, H, \mathcal{A}),
\end{align*} which does not explicitly depend on the size of the state space. 
\end{proof}
















==> app_ridge_linear_regression.tex <==
%!TEX root = appendix.tex
Below we give a general analysis of Ridge linear regression which is constantly used in the analysis of constrained linear MDPs above. 

Consider a dataset $\{x_i, y_i\}_{i=1}^N$ with $x_i\in\mathbb{R}^{d_1}$ and $y_i\in\mathbb{R}^{d_2}$ with $(x_i,y_i)$ being i.i.d sampled from some distribution $\nu$. We consider \emph{Ridge Linear Regression}:
\begin{align}
\label{eq:ridge_lr}
\hat{A}_N = \arg\min_{A\in\mathbb{R}^{d_2\times d_1}} \sum_{i=1}^N \| A x_i - y_i \|_2^2 + \lambda \|A \|^2_{F},
\end{align} with $\lambda\in \mathbb{R}^+$.

\begin{lemma}[Sample Complexity of Ridge Linear Regression]
Consider the setting introduced above and the optimization from~\eqref{eq:ridge_lr}. We have:
\begin{align*}
\hat{A}_N =  Y X^{\top}  \left(XX^{\top} + \lambda\mathbf{I}\right)^{-1} = \sum_{i=1}^N  y_i x_i^{\top}\left( XX^{\top} + \lambda\mathbf{I} \right)^{-1}.
\end{align*} where $X = [ x_1, \dots, x_N] \in\mathbb{R}^{d_1\times N}$ and $Y = [ y_1,\dots, y_N] \in\mathbb{R}^{d_2\times N}$.

Further assume that the bays optimal $\Exp[ y | x] =  A x$ with $A\in\mathbb{R}^{d_2\times d_1}$ and $y_i = A x_i + \varepsilon_i$ with $\|\varepsilon\|_1 \leq \beta\in\mathbb{R}^+$ for all $i$, and $\|A_i\|_1 \leq 1$ for all $i$ where $A_i$ is the $i$-th column of $A$, and $\|x_i\|_2\leq 1$ for all $i$. Define $V_N = \sum_{i=1}^N x_ix_i^{\top} + \lambda\mathbf{I}$ and consider a finite class of functions $\mathcal{F} = \{f: \states\to [0,H] \}$. Then for any $x$ and $f\in\mathcal{F}$, with probability at least $1-\delta$, we have for any $N$:
\begin{align*}
&\left\| \sum_{i=1}^N x_i (\varepsilon_i \cdot f) \right \|_{V_N^{-1}}^2 \leq \beta^2H^2  d \log\left( (N+\lambda)/\delta \right) + \beta^2 H^2 \log(|\mathcal{F}|/\delta), \\  
&\left\lvert (\hat{A}_Nx) \cdot f - (A x) \cdot f \right\rvert \leq \| x\|_{V_N^{-1}}  \left( \sqrt{\lambda d}H + \beta H \sqrt{d  \log( (N+\lambda)/\lambda)}  + \beta H \sqrt{\log(|\mathcal{F}|)/\delta} \right).
\end{align*}

Regarding computation when $d_2 \gg d_1$ and $d_2 \gg N$, computing $(\hat{A}_n x)\cdot f$ is $O(N)$ number of  queries of the inner product $\langle y, f \rangle$. 
\label{lemma:linear_regression}
\end{lemma}

\begin{proof}
The closed form of $\hat{A}$ can be verified by taking the derivative of Eq.~\ref{eq:ridge_lr} with respect to $A$, setting it to zero, and solving for $A$.  Below we focus on proving the statistical performance of ridge regression.   For notation simplicity, we ignore the subscript $N$ on $\hat{A}$ below. 

Denote $y_i = \varepsilon_i +  \Exp[y | x_i] = \varepsilon_i + Ax_i$. Using the closed-form of $\hat{A}$, we have:
\begin{align*}
&\hat{A} - A = \sum_{i=1}^N y_i x_i^{\top}\left( XX^{\top} + \lambda\mathbf{I} \right)^{-1} - A \\
& = \sum_{i=1}^N ( \varepsilon_i + A x) x_i^{\top}\left( XX^{\top} + \lambda\mathbf{I} \right)^{-1} -  A = \sum_{i = 1}^{N} \varepsilon_i x_i^{\top} (XX^{\top} + \lambda\mathbf{I})^{-1} + A XX^{\top}(XX^{\top}+\lambda\mathbf{I})^{-1} - A \\
& =   \sum_{i = 1}^{N} \varepsilon_i x_i^{\top}(XX^{\top} +\lambda\mathbf{I})^{-1} - \lambda A(XX^{\top}+\lambda \mathbf{I})^{-1}
\end{align*} Hence, for any $x$ and $f$, recall the definition of $V = XX^{\top} + \lambda\mathbf{I}$, we have:
\begin{align*}
&((\hat{A} - A)x) \cdot f = \sum_{i=1}^N   x^{\top} V^{-1} x_i \varepsilon_i^{\top} f - \lambda x^{\top} V^{-1} A^{\top} f 
\end{align*}
Let us bound the first term on the RHS of the above equality. 
\begin{align*}
\left\lvert \sum_{i=1}^N   x^{\top} V^{-1} x_i \varepsilon_i^{\top} f \right\rvert^2 \leq \| x \|_{V^{-1}}^2   \left\| \sum_{i=1}^N x_i (\varepsilon_i \cdot f) \right \|_{V^{-1}}^2
\end{align*} Using Lemma~\ref{lemma:self_normalized} and the fact that $ \left\lvert\varepsilon_i \cdot f \right\vert \leq  \|\varepsilon_1\|_1 \| f \|_{\infty} \leq \beta H$, we have that with probability at least $1-\delta$,  for any $n$, 
\begin{align*}
&  \left\| \sum_{i=1}^N x_i (\varepsilon_i \cdot f) \right \|_{V^{-1}}^2 \leq \beta^2H^2 \log\left( \det(V)^{1/2} \det(\lambda\mathbf{I})^{-1/2} /\delta \right).
\end{align*}
Apply a union bound over all $f\in\mathcal{F}$, we have that with probability at least $1-\delta$, for any $f\in\mathcal{F}$:
\begin{align*}
& \left\| \sum_{i=1}^N x_i (\varepsilon_i \cdot f) \right \|_{V^{-1}}^2 \leq \beta^2H^2 \log\left( \det(V)^{1/2} \det(\lambda\mathbf{I})^{-1/2} |\mathcal{F}| /\delta \right) \\
& = \beta^2H^2 \log(\det(V_N)^{1/2} \det(\lambda\mathbf{I})^{-1/2}) + \beta^2H^2\log(|\mathcal{F}|/\delta)\\
& \leq \beta^2H^2  d \log\left( (N+\lambda)/\delta \right) + \beta^2 H^2 \log(|\mathcal{F}|/\delta). 
\end{align*}

For the term $\lambda x^{\top} V^{-1} A^{\top} f$, we have that:
\begin{align*}
\left(\lambda x^{\top} V^{-1} A^{\top} f\right)^2 \leq \lambda^2 \| x \|_{V^{-1}}^2 \| A^{\top} f \|_{V^{-1}}^2 \leq \lambda^2 \|x\|_{V^{-1}} \frac{1}{\lambda} d H^2 = \lambda dH^2 \|x\|^2_{V^{-1}},
\end{align*} where we use the fact that $V_n^{-1}$ has the largest eigen-value being upper bounded by $1/\lambda$, and $\| A^{\top} f\|^2_2 \leq  = \sum_{i=1}^d (A_i\cdot f)^2 \leq d \|A_i\|^2_1 \|f\|^2_{\infty} \leq  dH^2$.


Regarding computation, using the notation of $\hat{A}$, we have $(\hat{A} x) \cdot f = x^{\top} \left( XX^{\top}+\lambda \mathbf{I} \right)^{-1} \sum_{i=1}^N x_i \left( y_i \cdot f\right)$.  Hence, Note that $x\in\mathbb{R}^{d_1}$. Hence the total computation complexity is $O( Nd_1^2 + N)$ which has nothing to do with $d_2$ assuming the query of inner product $\langle y, f\rangle$ is $O(1)$.
\end{proof}






